Secure Software Development Methodologies: A Multivocal Literature Review

In recent years, the number of cyber attacks has grown rapidly. An effective way to reduce the attack surface and protect software is adoption of methodologies that apply security at each step of the software development lifecycle. While different methodologies have been proposed to address software security, recent research shows an increase in the number of vulnerabilities in software and data breaches. Therefore, the security practices incorporated in secure software development methodologies require investigation. This paper provides an overview of security practices involved in 28 secure software development methodologies from industry, government, and academia. To achieve this goal, we distributed the security practices among the software development lifecycle stages. We also investigated auxiliary (non-technical) practices, such as organizational, behavioral, legal, policy, and governance aspects that are incorporated in the secure software development methodologies. Furthermore, we explored methods used to provide evidence of the effectiveness of the methodologies. Finally, we present the gaps that require attention in the scientific community. The results of our survey may assist researchers and organizations to better understand the existing security practices integrated into the secure software development methodologies. In addition, our bridge between "technical" and "non-technical" worlds may be useful for non-technical specialists who investigate software security. Moreover, exploring the gaps that we found in current research may help improve security in software development and produce software with fewer number of vulnerabilities.

==> all_practices.tex <==
\begin{table}[h]
  \centering
  \caption{All security practices involved in the project inception phase}
  \label{projectinception}
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{p{15em}p{15em}l} \hline
    \rowcolor{gray!50}
    Practices of the project inception phase & \multicolumn{1}{l}{Methodology} & \multicolumn{1}{l}{Reference} \\ \hline
    Define metrics and compliance reporting  & Microsoft SDL & \cite{howard2006security},\cite{whitepapermicrosoft},\cite{microsoftsdl}  \\ \hline
    Identify user roles and source capabilities & CLASP & \cite{web:lang:stats} \\ \hline
    Acquisition & NIST 800-160 & \cite{NIST2016volume1} \\ \hline
    Stakeholders needs and requirements definition & NIST 800-160 & \cite{NIST2016volume1} \\ \hline
    Business or mission analysis & NIST 800-160 & \cite{NIST2016volume1} \\ \hline
    Project planning & NIST 800-160 & \cite{NIST2016volume1} \\ \hline
    Personnel are accountable for software security & BSA & \cite{bsa2020} \\ \hline
    Forming the security team & Jones & \cite{jones2004secure} \\ \hline
    Identify security and privacy expert  & SDL-Agile & \cite{whitepapermicrosoft} \\ \hline
    \end{tabular}%
\end{table}%


\begin{table}[h]
  \centering
  \caption{All security practices involved in the analysis and requirements phase}
  \label{requirementphase}
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{p{15em}p{15em}l}
    \rowcolor{gray!50}
    Practices of the analysis and requirements phase & Methodology & \multicolumn{1}{l}{Reference} \\
    Define security requirements & All methodologies &  \\ 
    \multicolumn{1}{l}{Abuse and misuse cases} & Touchpoints, CLASP, Malaysia, ISDF, Khan, Daud & \cite{mcgraw2006software}, \cite{web:lang:stats}, \cite{malaysia2015}, \cite{alkussayer2010isdf}, \cite{khan2011secure}, \cite{daud2010secure} \\
    \multicolumn{1}{l}{Risk analysis} & Touchpoints, Grip on SSD, Khan, Farhan and Mostafa & \cite{mcgraw2006software},\cite{griponssd2015},\cite{khan2011secure},\cite{farhan2018methodology} \\
    Specify operational environment & CLASP & \cite{web:lang:stats}\\
    Identify user roles and resource capabilities & CLASP & \cite{web:lang:stats} \\
    Document security requirements & CLASP & \cite{web:lang:stats} \\
    Risk assessment & Singapore, SAP, Cisco, Citrix, SSDLC, Jones and Rastogi, Apvrille and Pourzandi, ISDF & \cite{csa2017},\cite{sap2020},\cite{cisco2021},\cite{citrix2021},\cite{isaca},\cite{jones2004secure},\cite{apvrille2005secure},\cite{alkussayer2010isdf} \\
    Security evaluation & Singapore & \cite{csa2017} \\
    Security control definition & SAFECode & \cite{safecode2018} \\
    Understanding adversaries & Google & \cite{viega2001building} \\
    Data classification & Malaysia & \cite{malaysia2015} \\
    Security planning & SAP   & \cite{sap2020} \\
    Data protection compliance evaluation & SAP   & \cite{sap2020} \\
    Gap analysis & Cisco & \cite{cisco2021} \\
    Privacy assessment & Cisco & \cite{cisco2021} \\
    Risk modeling & NIST 800-218 & \cite{nist218} \\
    Security constraints & SAFECode, Malaysia, SSDLC & \cite{safecode2018},\cite{malaysia2015},\cite{isaca} \\
    Feasibility study & SSDLC & \cite{isaca} \\
    Asset identification and valuation & Jones and Rastogi & \cite{jones2004secure} \\
    Threat model & Apvrille and Pourzandi, SSDM & \cite{sodiya2006towards} \\
    Quality gates & ISDF  & \cite{alkussayer2010isdf} \\
    User stories & Daud, GE & \cite{daud2010secure},\cite{ge} \\
    Application portfolio analysis & Farhan and Mostafa & \cite{farhan2018methodology} \\
    User risk analysis & Farhan and Mostafa & \cite{farhan2018methodology} \\
    Review design & GE    & \cite{ge} \\
    Provide security design input & GE    & \cite{ge} \\
    Evaluate security specification & Singapore & \cite{csa2017}\\
    \end{tabular}%
\end{table}%


\begin{table}[h]
  \centering
  \caption{All security practices involved in the architectural and detailed design stage}
  \label{design}
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{p{15em}p{15em}p{12em}}
    \rowcolor{gray!50}
    Practices of the design phase & Methodology & \multicolumn{1}{l}{Reference} \\
    Architecture and design definition	 & All practices &  \\
    Design requirements & MS SDL & \cite{microsoftsdl} \\
    Threat modeling & MS SDL, SAFECode, Malaysia, BSA, Cisco, Citrix, Jones and Rastogi, ISDF, Daud, Khan, SDL-Agile & \cite{microsoftsdl},\cite{safecode2018},\cite{malaysia2015},\cite{bsa2020},\cite{cisco2021},\cite{citrix2021},
    \cite{jones2004secure},\cite{alkussayer2010isdf},\cite{daud2010secure},\cite{khan2011secure},\cite{whitepapermicrosoft} \\
    Architecture and design risk analysis & Touchpoints, BSA, ISDF, Farhan and Mostafa& \cite{mcgraw2006software},\cite{bsa2020},\cite{alkussayer2010isdf}, \cite{farhan2018methodology} \\
    Identify attack surface & CLASP & \cite{web:lang:stats} \\
    Specify database security configuration & CLASP & \cite{web:lang:stats}  \\
    Annotate class designs with security properties & CLASP & \cite{web:lang:stats} \\
    Apply security principles to design & CLASP, SAFECode, Google, Malaysia, BSA, NIST 800-218, Chatterjee and De & \cite{web:lang:stats},\cite{safecode2018},\cite{viega2001building},\cite{malaysia2015}, \cite{bsa2020},\cite{nist218},\cite{chatterjee2013framework} \\
    Critical security architectural and design review & Singapore, SAFECode, NIST 800-218, Jones and Rastogi, Pourzandi, Khan, SDL-Agile &  \cite{csa2017},\cite{safecode2018},\cite{NIST2016volume1},\cite{jones2004secure},\cite{khan2011secure},\cite{whitepapermicrosoft}\\
    Develop an encryption strategy & SAFECode & \cite{safecode2018} \\
    Standardize identity and access management & SAFECode & \cite{safecode2018} \\
    Establish log requirements and audit practices & SAFECode & \cite{safecode2018} \\
    Use of assurance measures & BSA   & \cite{bsa2020} \\
    Protect all forms of code from unauthorized access and tampering & NIST 800-218 & \cite{nist218} \\
    Security constraints & Malaysia, Chatterjee and De & \cite{malaysia2015},\cite{chatterjee2013framework} \\
    Risk assessment & Malaysia & \cite{malaysia2015} \\
    Risk mitigation & Jones and Rastogi & \cite{jones2004secure} \\
    Security specifications & SSDM  & \cite{sodiya2006towards} \\
    Review security specifications & SSDM  & \cite{sodiya2006towards} \\
    Security toolkits selection & ISDF  &  \cite{alkussayer2010isdf}\\
    Use cases & Daud  & \cite{daud2010secure}  \\
    Update threat model & SDL-Agile, GE & \cite{whitepapermicrosoft},\cite{ge} \\
    Communicate privacy-impact design changes to the team privacy advisor & SDL-Agile & \cite{whitepapermicrosoft} \\
    Update security user stories & GE    & \cite{ge} \\
    Attack surface analysis review and reduction & GE    & \cite{ge} \\
    Review security controls & Singapore & \cite{csa2017}\\
    \end{tabular}%
\end{table}%


\begin{table}[h]
  \centering
  \caption{All security practices involved in implementation phase}
  \label{implementation}
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{p{15em}p{15em}p{10em}}
        \rowcolor{gray!50}
    Practices of implementation phase & Methodology & \multicolumn{1}{l}{Reference} \\
    Define and use cryptographic services & MS SDL &  \\
    \multicolumn{1}{l}{SAST} & MS SDL, SAFECode, SAP, Cisco, Citrix, ISDF, Khan, Farhan and Mostafa, GE & \cite{microsoftsdl},\cite{safecode2018},\cite{sap2020},\cite{cisco2021},\cite{citrix2021}, \cite{alkussayer2010isdf},\cite{khan2011secure},\cite{farhan2018methodology},\cite{ge} \\
    \multicolumn{1}{l}{Use approved tools} & MS SDL & \cite{microsoftsdl} \\
    \multicolumn{1}{l}{Code review} & Touchpoints, Grip on SSD, Singapore, BSA, SAP, Citrix, NIST 800-218, ISDF, Khan & \cite{mcgraw2006software},\cite{griponssd2015},\cite{csa2017},\cite{bsa2020}, \cite{sap2020},\cite{citrix2021},\cite{nist218},\cite{alkussayer2010isdf},\cite{khan2011secure}\\
    Integrate security analysis into source management process & CLASP & \cite{web:lang:stats} \\
    \multicolumn{1}{l}{Implement interface contracts} & CLASP & \cite{web:lang:stats} \\
    Implement and elaborate resource policies and security technologies & CLASP & \cite{web:lang:stats}\\
    \multicolumn{1}{l}{Implementation} & NIST 800-160 & \cite{NIST2016volume1} \\
    Integration & NIST 800-160 & \cite{NIST2016volume1} \\
    \multicolumn{1}{l}{Handle data safely} & SAFECode & \cite{safecode2018} \\
    Handle errors & SAFECode & \cite{safecode2018} \\
    \multicolumn{1}{l}{Use safe functions only} & SAFECode & \cite{safecode2018} \\
    Use coding best practices and standards & Google, BSA, NIST 800-218, SSDLC,Jones and Rastogi, ISDF, Khan, Farhan and Mostafa, SDL-Agile & \cite{viega2001building},\cite{bsa2020},\cite{nist218},\cite{isaca},\cite{jones2004secure}, \cite{alkussayer2010isdf},\cite{khan2011secure},\cite{farhan2018methodology},\cite{whitepapermicrosoft} \\
    Use of advanced mitigation strategies & Google & \cite{viega2001building} \\
    Common software vulnerabilities and controls (about secure coding practices) & Malaysia, BSA, Daud & \cite{malaysia2015},\cite{bsa2020},\cite{daud2010secure} \\
    Secure software processes (Code review, SAST, DAST, unit tests, integration tests,regression tests ) & Malaysia & \cite{malaysia2015} \\
    Securing build environments (ACLs, code signing) & Malaysia, BSA & \cite{malaysia2015}, \cite{bsa2020} \\
    Log implementation & BSA   & \cite{bsa2020} \\
    Secure code repositories (about peer-review code) & Cisco & \cite{cisco2021} \\
    Secure modules & Cisco, Daud & \cite{cisco2021},\cite{daud2010secure} \\
    Security regression testing & Citrix & \cite{citrix2021} \\
    Variant Analysis & Citrix & \cite{citrix2021} \\
    Cognizance of security risks & Jones and Rastogi & \cite{jones2004secure} \\
    Security safeguards & Jones and Rastogi & \cite{jones2004secure} \\
    DAST  & ISDF, GE & \cite{alkussayer2010isdf},\cite{ge} \\
    Data protection services & Chatterje, Gupta, and De & \cite{chatterjee2013framework} \\
    Secure document delivery & Chatterje, Gupta, and De & \cite{chatterjee2013framework} \\
    Application security integration & Chatterje, Gupta, and De & \cite{chatterjee2013framework} \\
    Fix all issues identified by code analysis tools for unmanaged code & SDL-Agile & \cite{whitepapermicrosoft} \\
    Open source vulnerability assessment & GE    & \cite{ge} \\
    Source-level security review & CLASP & \cite{web:lang:stats}\\
    \end{tabular}%
\end{table}%


\begin{table}[h]
  \centering
  \caption{All security practices involved in the verification and testing phase}
  \label{testing}
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{p{15em}p{15em}p{10em}}
    \rowcolor{gray!50}
    Verification and testing phase & Methodology & \multicolumn{1}{l}{Reference} \\
    Automated tasting (DAST, SAST) & MS SDL, SAFECode, Google, SAP, ISDF & \cite{microsoftsdl},\cite{safecode2018},\cite{viega2001building},\cite{sap2020},\cite{alkussayer2010isdf} \\
    Penetration testing & MS SDL, Touchpoints, Singapore, Cisco, Citrix, Jone and Rastogi, SSDM, ISDF, Daud, Farhan and Mostafa, GE & \cite{microsoftsdl},\cite{mcgraw2006software},\cite{csa2017},\cite{cisco2021},\cite{citrix2021}, \cite{jones2004secure},\cite{sodiya2006towards},\cite{alkussayer2010isdf},\cite{daud2010secure},\cite{farhan2018methodology},\cite{ge} \\
    Risk analysis & Touchpoints & \cite{mcgraw2006software} \\
    identify, implement, and perform security tests & CLASP, Grip on SSD & \cite{web:lang:stats},\cite{griponssd2015} \\
    Verify security attributes of resources & CLASP, Grip on SSD, NIST 800-218 & \cite{web:lang:stats},\cite{griponssd2015},\cite{nist218} \\
    Verification and validation (vulnerability, penetration, abuse and misuse) & NIST 800-160, SAP, SDL-Agile & \cite{NIST2016volume1},\cite{sap2020},\cite{whitepapermicrosoft} \\
    Application security testing & Singapore & \cite{csa2017} \\
    System security testing & Singapore, Apvrille and Pourzandi & \cite{csa2017},\cite{apvrille2005secure} \\
    Manual testing(penetration testing, verification) & SAFECode & \cite{safecode2018} \\
    Unit testing & Google, SSDLC, Jones and Rastogi, Apvrille and Pourzandi, Daud & \cite{viega2001building},\cite{isaca},\cite{jones2004secure},\cite{apvrille2005secure},\cite{daud2010secure} \\
    Integration testing & Google, SSDLC, Jones and Rastogi & \cite{viega2001building},\cite{isaca},\cite{jones2004secure} \\
    Investigating systems & Google & \cite{viega2001building} \\
    Attack surface validation & Malaysia, BSA & \cite{malaysia2015},\cite{bsa2020} \\
    Test data management & Malaysia & \cite{malaysia2015} \\
    Security control testing & BSA   & \cite{bsa2020} \\
    Adversarial security testing techniques & BSA   & \cite{bsa2020} \\
    Open-source known vulnerability scans & SAP   & \cite{sap2020} \\
    Vulnetability testing & Cisco, Apvrille and Pourzandi & \cite{cisco2021},\cite{apvrille2005secure} \\
    Privacy control validation & Cisco & \cite{cisco2021} \\
    Security regression testing & Citrix & \cite{citrix2021} \\
    Vulnerability assessment & Citrix, Apvrille and Pourzandi, Chatterje, Gupta, and De & \cite{citrix2021},\cite{apvrille2005secure},\cite{chatterjee2013framework} \\
    Automated variant analysis & Citrix & \cite{citrix2021} \\
    Test executable code (functional, dynamic, fuzz, penetration) & Citrix, ISDF, Daud & \cite{citrix2021},\cite{alkussayer2010isdf},\cite{daud2010secure} \\
    Code review(SAST, manual, open-source components) & SSDLC, Apvrille and Pourzandi & \cite{isaca},\cite{apvrille2005secure} \\
    Certification & Jones and Rastogi & \cite{jones2004secure} \\
    Threat-based testing & ISDF, Khan & \cite{alkussayer2010isdf},\cite{khan2011secure} \\
    Code integrity and handling & ISDF  & \cite{alkussayer2010isdf} \\
    Scurity test cases & Khan  & \cite{khan2011secure} \\
    Security assessment & Chatterje, Gupta, and De & \cite{chatterjee2013framework}\\
    Security audit and review & Chatterje, Gupta, and De, Farhan and Mostafa & \cite{chatterjee2013framework},\cite{farhan2018methodology} \\
    Security metrics development & Farhan and Mostafa & \cite{farhan2018methodology} \\
    \end{tabular}%
\end{table}%

==> table.tex <==
\begin{figure}[t]
\label{picture1}
    \includegraphics[width=1\textwidth]{Timeline.png}
    \caption{The timeline}
\end{figure}

\begin{landscape}
\tiny % text size
\renewcommand{\arraystretch}{0.8}%for the length between lines
\setlength{\tabcolsep}{2pt}%the gap width of columns
\setlength\LTcapwidth{\textwidth} % default: 4in (rather less than \textwidth...)      
\setlength\LTleft{0pt}            % default: \fill don't know use or not
\setlength\LTright{0pt}           % default: \fill  don't know use or not

%\begin{longtable}{|p{1.5cm}|ccccccc|p{1cm}|cccccccc|} I don't know what is better to use
\begin{longtable}{@{\extracolsep{\fill}}|c|ccccccc|c|ccccccc|} 
\caption{Summary of secure SDLC methodologies and involved secure practices}
\label{tab:waterfall}\\ 
\hline
\multirow{3}{*}{Methodology} & \multicolumn{7}{c|}{Organizational-wide processes}  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Processes\\ that\\ cover all\\ stages\\ of SDLC\end{tabular}} & \multicolumn{7}{c|}{\multirow{2}{*}{SDLC stages for a specific project}}\\ \cline{2-8} & \multicolumn{2}{c|}{Technical process}& \multicolumn{3}{c|}{Technical management process}
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Organizational processes\end{tabular}} &   & \multicolumn{7}{c|}{}  \\ \cline{2-8} \cline{10-16}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}During \\ all \\ stages\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Preliminary\\ stages\\ for \\ maintenance\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Risk\\manage-\\ment\\frame-\\work\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Third\\party\\compo-\\nents\\manage-\\ment\end{tabular}} & \multicolumn{1}{c|}{Other} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Security\\ culture\end{tabular}}      & Other   &     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Project\\ inception\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Analysis \\ and \\ requirements\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Architectural \\ and detailed \\ design\end{tabular}} & \multicolumn{1}{c|}{Implementation} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Verification \\ and testing\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Release \\ and \\ maintenance\end{tabular}} & Disposal \\ \hline
%\endfirsthead % repeat header
%
\endhead
%
\multicolumn{16}{|c|}{Industry and government methodologies} \\ \hline
\makecell {MS SDL\\ \cite{howard2006security},\cite{whitepapermicrosoft},\cite{microsoftsdl}  \\ (2006)} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Define \\ and publish\\ a list of\\ approved\\ tools \\ \textbullet Define\\ and use\\ cryptographic\\ standards\\ \textbullet Tracking\\ factors\\ that\\ influence \\ security \\ requirements \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Establish\\ a standard\\ incident\\ response\\ process \\ \end{tabular}}   
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\checkmark{}} 
&\multicolumn{1}{c|}{}    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Provide\\ training\\ \end{tabular}} 
&  
&   
&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Define metrics\\ and \\compliance \\ reporting \end{tabular}}  &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Define security\\ requirements \end{tabular}} &\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Establish design\\ requirements\\ \textbullet Threat\\ modeling\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Define and use\\ cryptographic\\ standards\\ \textbullet SAST\\ \textbullet Use approved\\ tools\end{tabular}} 
&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet DAST\\ \textbullet Penetration\\ testing\\\end{tabular}} 
& \multicolumn{1}{c|}{} 
&  \\ \hline


\makecell {Touchpoints\\ \cite{mcgraw2006software}\\ (2006)}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Guidelines,\\ principles\\ and rules\\ \end{tabular}} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\checkmark{}} 
& \multicolumn{1}{c|}{}
&\multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Knowledge\\ manage-\\ment and \\ training \\ \end{tabular}}    
&  
& \begin{tabular}[c]{@{}l@{}} External\\ review \\ \end{tabular}  
& \multicolumn{1}{c|}{}  
&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Abuse cases \\ \textbullet Security\\ requirements\\ \textbullet Architectural\\ risk analysis \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Architectural\\ risk analysis \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Code review\\ (tools)\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk analysis \\ \textbullet Penetration\\ testing\\\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Penetration\\ testing\\ \textbullet Security\\ operations\end{tabular}} 
& \\ \hline


\makecell {CLASP\\ \cite{web:lang:stats}\\ (2006)}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Identify\\ global\\ security\\ policy\end{tabular}} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Research\\ and\\ assess\\ security\\ posture\\ of\\techno-\\logy \\solutions \end{tabular}} 
& \multicolumn{1}{c|}{}  
&\multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Institute\\ security\\ awareness\\program\end{tabular}} 
&  
& \begin{tabular}[c]{@{}l@{}}Monitor\\ security\\ metrics\\ \end{tabular}   
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Specify\\ operational\\ environment \\ \textbullet Identify user\\roles and \\ resource \\ capabilities\\ \textbullet Document\\ security-relevant\\ requirements\\ \textbullet Misuse cases\\ \end{tabular}}    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Identify\\ resources\\ and trust\\ boundaries\\ \textbullet Identify\\ attack surface\\ \textbullet Specify\\ database\\ security\\ configuration\\ \textbullet Annotate\\ class designs\\ with security\\ properties\\ \textbullet Apply security\\ principles\\ to design \\ \textbullet Threat modeling\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Integrate\\ security analysis\\ into source\\ management\\ process\\ \textbullet Implement\\ interface\\ contracts\\ \textbullet Implement\\ and elaborate\\ resource policies\\ and security\\ technologies\\ \textbullet Address reported\\ security issues\\\textbullet Source-level\\ security review \end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Identify,\\ implement,\\ and perform\\ security tests\\ \textbullet Verify\\ security\\ attributes\\ of resources\\ \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Code signing\\ \textbullet Build\\ operational\\ security guide\\ \textbullet Manage\\ security issue\\ disclosure \\process\\ \end{tabular}} 
& \\ \hline

\makecell {Grip on SSD \\\cite{griponssd2015}\\ (2015)}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Set up\\standard\\ security\\requirements\\ \textbullet Maintain\\standard\\security\\requirements\\ \textbullet Business\\ impact\\ analysis\end{tabular}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}   
& \multicolumn{1}{c|}{} 
&  
& \begin{tabular}[c]{@{}l@{}}Risk\\ control\\ and risk\\acceptance \end{tabular} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Risk analysis \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ test plans\end{tabular}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Code reviews\\ \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security testing\\ \textbullet Penetration\\ testing \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk acceptance\\ \textbullet Maturity\\ guidance\\ \textbullet Provide\\ accountability \end{tabular}} 
&  \\ \hline


\makecell {NIST 800-160 \\ \cite{NIST2016volume1} \\ (2016)}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\checkmark{}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Deci-\\sion\\manage-\\ment\\ \textbullet Confi-\\guration\\manage-\\ment\\ \textbullet Infor-\\mation\\manage-\\ment\\ \textbullet Measu-\\rement \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Knowledge\\manage-\\ment\end{tabular}} 
& \begin{tabular}[c]{@{}l@{}}\textbullet Lifecycle\\model\\management\\\textbullet Infra-\\structure\\management\\ \textbullet Portfolio\\management\\ \textbullet Human\\resource\\management\\ \textbullet Quality\\management \end{tabular} 
& \begin{tabular}[c]{@{}l@{}}\textbullet Project\\assessment\\and control\\ \textbullet Quality\\assurance\\ \textbullet System\\analysis \end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Aquisition\\ \textbullet Stakeholder\\needs and\\requirements\\definition\\ \textbullet Business\\ or mission\\ analysis\\ \textbullet Project\\ planning \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet System\\ requirements\\defenition \end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Architecture\\definition\\ \textbullet Design definition \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Implementation\\ \textbullet Integration \end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Verification\\ \textbullet Validation\\\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Transition\\ \textbullet Operation\\ \textbullet maintenance\\ \textbullet Supply \end{tabular}} 
& \checkmark{}\\ \hline



\makecell {Singapore \\ \cite{csa2017}\\ (2017)}
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\checkmark{}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{} 
&    
&   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ planning\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Systems\\ security\\ classification\\ \textbullet  Risk\\ assessment\\ \textbullet Threat and risk\\assessment\\\textbullet Define security\\ requirements\\ for tender\\\textbullet Evaluate\\ security\\ specification\\\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Review\\security\\ architecture\\\textbullet Review\\ security controls\\\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Code review  \end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Application\\security texting\\ \textbullet System\\security texting\\\textbullet Penetration\\ testing\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security review\\ \textbullet Configuration\\management\\ \textbullet Change \\management\\ \textbullet Continuous\\monitoring\end{tabular}} 
& \checkmark{}  \\ \hline


\makecell {SAFECode\\ \cite{safecode2018}\\ (2018)}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Establish\\ coding\\ standards\\ and\\ conventions\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Define\\ internal\\ and external\\ policies of\\ vulnerability\\ disclosure\\ \textbullet Define\\ roles and\\ responsibilities\\ of\\ vulnerability\\ disclosure \end{tabular}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\checkmark{} \end{tabular}} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{}  
& \begin{tabular}[c]{@{}l@{}}Planning\\ the\\ implemen-\\tation\\ and\\ deploy-\\ment\\ of secure\\ develop-\\ment\end{tabular}  
& 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Application\\ security control\\ definition\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Follow the secure\\ design principles\\ \textbullet Threat modeling\\ \textbullet Perform\\ architectural\\ and design reviews\\ \textbullet Develop\\ an encryption\\ strategy\\ \textbullet Standardize\\identity and access\\ management\\ \textbullet Establish\\ log requirements\\ and audit practices\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Handle data\\ safely\\ \textbullet Use safe\\ functions only\\ \textbullet Use code analysis\\tools\\ \textbullet Handle errors\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Automated\\ testing\\ \textbullet Manual\\ testing\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Fix the\\ vulnerability\\\textbullet Vulnerability\\ disclosure\\ \textbullet Manage\\ vulnerability\\ reporters\\ \textbullet Secure\\ development\\ lifecycle\\ feedback\end{tabular}} 
&  \\ \hline


\makecell {Google \\ \cite{adkins2020building} \\ (2020)}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Disaster\\planning\\ \textbullet Recovery\\ planning\\ \textbullet OpSec plan\end{tabular}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Crisis\\ manage-\\ment\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Build\\ a culture\\ of security\\ and\\ reliability\end{tabular}}  
& \begin{tabular}[c]{@{}l@{}}Under-\\standing\\ roles and\\ responsi-\\bilities\end{tabular}
&  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Understanding\\ adversaries\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Design tradeoffs\\ \textbullet Design for least\\ privilege\\ \textbullet Design for\\ understandability\\ \textbullet Design for\\ a changing\\ landscape\\ \textbullet Design for\\ resilience\\ \textbullet Design for\\ recovery\\ \textbullet Mitigating\\ Denial-of-Service\\ attacks\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Deploying code\\ using\\ best practices\\ \textbullet Use of advanced\\ mitigation\\ strategies\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Unit testing\\\textbullet Integration\\testing\\ \textbullet Dynamic\\ program analysis\\ \textbullet Fuzz testing\\ \textbullet Static\\program analysis\\ \textbullet Investigating\\ systems\\ \end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Recovery and\\ aftermath\\ \textbullet Crisis\\  management\end{tabular}}  
& \\ \hline


\makecell {Malaysia \\ \cite{malaysia2015}\\ (2020)} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Develop\\ end-of-life\\ policies\end{tabular}} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{}  
&   
&   
& \multicolumn{1}{c|}{}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Sources\\ of security\\ requirements\\ \textbullet Data\\ classification\\ \textbullet Use case\\ and misuse case\\ modeling\\\textbullet Risk management\end{tabular}}     
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ design\\ considerations\\ \textbullet Additional\\ design\\ configurations\\ \textbullet Threat modeling\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Common\\ security\\ vulnerabilities\\ and controls\\ \textbullet Secure software\\ processes\\ \textbullet Securing\\ build\\ environments\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Attack surface\\ validation\\ \textbullet Test data\\ management\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Software\\ acceptance\\ considerations\\ \textbullet Verification\\ and validation\\ \textbullet Certification\\ and accreditation\\ \textbullet Installation\\ \textbullet Operation,\\ monitor and\\ maintenance\\ \textbullet Incident\\ management\\ \textbullet Problem\\ management\\ \textbullet Change\\ management\end{tabular}} 
& \checkmark{}  \\ \hline


\makecell {BSA\\ \cite{bsa2020} \\ (2020)}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Create and\\ maintain\\ software\\ development\\ environment\\ \textbullet Identification\\ of coding\\ standards\\\end{tabular}}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\checkmark{}} 
& \multicolumn{1}{c|}{\checkmark{}} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\training\end{tabular}}  
& \begin{tabular}[c]{@{}l@{}}Personnel\\ are\\ account-\\able\\ for\\ software\\ security\end{tabular}
& \begin{tabular}[c]{@{}l@{}}\textbullet Secure\\ development\\ processes\\ are\\ documented\\ \textbullet Identity\\ and access\\ management\end{tabular} 
& \multicolumn{1}{c|}{}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security \\ requirements\\are gathered\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Threat modeling\\ and risk analysis\\ \textbullet Use of assurance\\ measures\\ \textbullet Design for\\ least privilege\\ \textbullet Design for\\ authorization\\ and access control\\ \textbullet Ensure\\security\\capabilities\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure coding\\ practices\\ \textbullet Known\\ vulnerabilities,\\ unsafe functions,\\ unsafe libraries\\ \textbullet Code review\\ \textbullet Log implementation\\ \textbullet Measures to\\prevent\\counterfeiting\\and tampering\\ \textbullet Proper usages of\\software are\\established\\\textbullet Software is\\identifiable\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Analysis and\\ validation of\\ attack surface\\ \textbullet Software\\ security controls\\ are tested\\ \textbullet Adversarial\\ security\\ testing\\ techniques\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Vulnerability\\ notification\\ and patching\\ \textbullet Vulnerability\\ management\\ \textbullet Configuration\\ guidance\\ \textbullet Maintenance\\ of lifecycle\\ guidance\end{tabular}}   
&    \\ \hline



\makecell {SAP\\ \cite{bsa2020} \\ (2020)} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\checkmark{}}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ training\end{tabular}}  
&  
&  
& \multicolumn{1}{c|}{}  
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Risk assessment\\ \textbullet Data protection\\ compliance evaluation\\ \textbullet Define the security\\ and privacy requirements\\ \textbullet Define security controls\end{tabular}} 
%& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Create and\\ maintain\\ a security plan\\ \textbullet Risk assessment\\ \textbullet Data protection\\ compliance\\ evaluation\\ \textbullet Design reviews\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Code reviews\\ \textbullet Static-code\\ analysis\\ \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet SAST\\ \textbullet DAST\\ \textbullet Open-Source\\ known\\ vulnerability\\ scans\\ \textbullet Security\\ validation\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ response\end{tabular}}  
&  \\ \hline



\makecell {Cisco\\ \cite{cisco2021} \\ (2021)} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\checkmark{}}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ training\end{tabular}} 
& 
& 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Gap analysis\\ and risk\\ assessment\\ \textbullet Security\\requirements\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Threat modelling\\ \end{tabular}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure modules\\ \textbullet Static analysis\\ \textbullet Secure code\\ repositories\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Vulnerability\\ and penetration\\ testing\\ \textbullet Privacy control\\validation\\ \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ and privacy\\ readiness\\ \textbullet Security and\\ operational\\ management\\ \textbullet Continuous\\ monitoring\\ and updates\\ \textbullet Maintaining\\ privacy controls \end{tabular}} 
& \\ \hline


\makecell {Citrix\\ \cite{citrix2021} \\ (2021)} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Bug bounty\\ \textbullet Red team\\ engagements\\ \textbullet Product-\\wide\\ pentests\\ \textbullet External\\ assessment\\ \textbullet CI/CD\\ pipeline\\ security\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Remediation\\ programs\end{tabular}} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\checkmark{}} 
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\training\end{tabular}}  
&   
&  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Planning and\\ requirement\\ gathering\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Threat modeling\end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Code review\\ \textbullet SAST\\ \textbullet Variant analysis\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ regression\\ testing\\ \textbullet Automated\\variant\\analysis\\ \textbullet Vulnerability\\assessment\\ \textbullet Feature\\ penetration\\ testing\end{tabular}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \textbullet Vulnerability\\ Response\\ \textbullet Product\\ Security\\ Incident\\ Response\\ \textbullet Logging and\\ monitoring\end{tabular}}  &  \\ \hline



\makecell {NIST 800-218\\ \cite{nist218} \\ (2022)} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Reuse\\ existing\\ software\\ \textbullet Implement\\ supporting\\ toolchains\\ \textbullet Implement\\ and\\ maintain\\secure\\ environments\\ \textbullet Define\\ security\\ requirements\end{tabular}}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Verify\\third-\\party\\software\\complies\\ with\\ security\\ require-\\ments\end{tabular}}   
& \multicolumn{1}{c|}{} 
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}l@{}}Implement roles and\\ responsibilities\end{tabular}}  

& \begin{tabular}[c]{@{}l@{}}Define\\ and use\\ criteria\\ for software\\ security\\ checks\end{tabular} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Configure the\\ compilation,\\ interpreter,\\ and build\\ processes\\ to improve\\ executable\\ security\end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Design software\\ to meet security\\ requirements\\ and mitigate\\ security risks\end{tabular}\footnote{This practice is about security requirement}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Configure\\ software to have\\ secure settings\\ by default\\ \textbullet Review the\\ software design\\ to verify\\ compliance\\ with security\\ requirements\\ and risk\\ information\\ \end{tabular}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Review and/or\\ analyze\\ human-readable\\ code\\  \textbullet Create source\\ code by adhering\\ to secure coding\\ practices\\ \textbullet Protect all forms\\ of code from\\ unauthorized\\ access and\\ tampering\end{tabular}}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Test executable\\ code\\ \end{tabular}}   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Provide a\\ mechanism \\for verifying \\software release\\ integrity\\\textbullet Archive and\\ protect each\\ software release\\ \textbullet Identify and \\confirm\\ vulnerabilities\\ on an ongoing basis\\ \textbullet Assess, prioritize,\\ and remediate\\ vulnerabilities\\ \textbullet Analyze\\ vulnerabilities\\ to identify their root\\ causes\end{tabular}} 
& \\ \hline

\makecell {SSDLC\\ \cite{isaca} \\ (Last\\ access\\ 2022)}                       
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{}                                                                         
&            
&                                                                                                         
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk assessment\\ \textbullet Security\\ constraints\\ \textbullet Feasibility\\ study and\\ requirements\\ validation\end{tabular}}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk assessment\\\textbullet Security\\ constraints\end{tabular}}                                                                                
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Apply\\ coding standards\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Code review\\ \textbullet Unit testing,\\ integration\\ testing\end{tabular}}                                                                    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Platform\\ security\\ \textbullet Penetration\\ testing\\ \textbullet Continuous\\ monitoring\end{tabular}}                                                                      
& \checkmark{}         \\ \hline


\multicolumn{16}{|c|}{Academy methodologies} \\ \hline


\makecell {Jones\\ and\\ Rastogi \\ \cite{jones2004secure}\\(2004)}                        
& \multicolumn{1}{c|}{}                                                               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Define\\ response\\ process\\ for handling\\security bugs\\ \textbullet Define\\ backup\\ procedures\\ \textbullet Define\\ business\\ continuity\\ procedures \end{tabular}}      
& \multicolumn{1}{c|}{\checkmark{}}                                                          
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ training\end{tabular}}                                                                        
&            
&                                                                                                         
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Forming\\ the security\\ team\end{tabular}}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk assessment\\ \textbullet Asset\\ identification\\ and validation\\ \textbullet Requirement\\ gathering\end{tabular}}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Threat modelling\\ \textbullet System design\\ \textbullet Security review\\ \textbullet Risk\\ mitigation\end{tabular}}                                                                                
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Cognizance\\ of security risks\\ \textbullet Secure coding\\ \textbullet Security\\ safeguards\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Unit testing\\ \textbullet Integration\\Quality\\ assurance\\ testing\\ \textbullet Penetration\\ testing\\ \textbullet Certification\end{tabular}}                                                                    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Patch\\ management\\ \textbullet Monitoring\end{tabular}}                                                                      
& \checkmark{}         \\ \hline



\makecell {Apvrille\\ and\\Pourzandi \\ \cite{apvrille2005secure} \\(2005)}                      
& \multicolumn{1}{c|}{}                                                             
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}     
& \multicolumn{1}{c|}{}                                                                        
&            
&                                                                                                         
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ environment\\ and objectives\\ description\\ \textbullet Threat modeling\\ \textbullet Security policy\\ \textbullet Risk evaluation\end{tabular}}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security design\\\textbullet Reviewing design\end{tabular}}                                                                               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ best practices \end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Peer review\\ \textbullet Unit testing\\ \textbullet System texting\\ \textbullet Evaluating bugs\end{tabular}}                                                                    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Operation\\ and\\ maintenance\end{tabular}}                                                                     
&          \\ \hline



\makecell {SSDM\\ \cite{sodiya2006towards}\\ (2006)}                   
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                 
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                              
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ training\end{tabular}}                                                                         
&           
&                                                                                                        
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Requirement\\ definition\\ \textbullet Threat modelling\end{tabular}}                                                                      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ specifications\\ \textbullet Review security\\ specifications\end{tabular}}                                                                                
& \multicolumn{1}{c|}{Coding}              
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Penetration\\ testing\end{tabular}}                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Implementation\\ and\\ maintenance\end{tabular}}                                                                     
&          \\ \hline


\makecell {ISDF \\ \cite{alkussayer2010isdf}\\(2010)}                         
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                              
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Education\\ and\\ awareness\end{tabular}}                                                                         
&           
&  \begin{tabular}[c]{@{}l@{}}External\\ reviews\end{tabular}                                                                                                      
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ requirements\\ \textbullet Abuse cases\\ \textbullet Quality gates\\ \textbullet Risk\\ assessment\end{tabular}}                                                                      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Risk analysis\\ \textbullet Threat modeling\\ \textbullet Security\\ toolkits\\ selection\end{tabular}}                                                                                     
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure coding\\ practices\\ \textbullet Static/dynamic\\ analysis tools\\ \textbullet Code review\\ (Manual)\\ \textbullet Logging and\\ tracing\end{tabular}}              
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Fuzz testing\\ \textbullet Penetration\\ testing\\ \textbullet Threat-based\\ testing\\ \textbullet Automated\\ testing tools\\ \textbullet Code integrity\\ and handling\end{tabular}}                                                                   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Final\\ security review\\ \textbullet Security feedback\\ \textbullet Response\\ execution\\ \textbullet Threat models\\ update\\ \textbullet Response\\ planning\\ \textbullet Release\\ preparation\end{tabular}}  
&          \\ \hline


\makecell {Daud\\ \cite{daud2010secure} \\(2010)}                        
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                          
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{}                                                                         
&            
&                                                                                                         
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet User Stories\\ \textbullet Security\\ functional\\ requirements\\ \textbullet Non-functional\\ security\\ requirements\\ \textbullet User\\ requirements\\ \textbullet Misuse cases\\ \textbullet Mitigation plan\end{tabular}}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Threat model\\ \textbullet Input data types\\ \textbullet Security use cases\end{tabular}}                                                                                
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security modules\\ \textbullet List of known\\ security\\ vulnerabilities\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Unit testing\\ \textbullet Functional\\ testing\\ \textbullet Penetration\\ testing\\ \textbullet Fuzz testing\end{tabular}}                                                                    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ measurement\\ \textbullet Monitoring\\ requirements\\ \textbullet Security\\ upgrade\end{tabular}}                                                                     
&          \\ \hline

\makecell {Khan \\ \cite{khan2011secure} \\ (2011)}                        
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                          
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{}                                                                         
&            
&                                                                                                         
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ requirement\\ identification\\ \textbullet Security\\ requirement\\ documentation\\ \textbullet Risk analysis\\ \textbullet Secure\\ requirement\\ review and\\ verification\end{tabular}}                                                                      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure design\\ architecture\\ \textbullet Threat modeling\\ \textbullet Secure design\\ documentation\\ \textbullet Review and\\ verification\\ of secure design\end{tabular}}                                                                                
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure code\\ writing\\ \textbullet Static analysis\\ \textbullet Code review\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Secure test\\ activities\\ \textbullet Security\\ test cases\end{tabular}}                                                                   
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security\\ monitoring\\ and create\\ a response plan\\ \textbullet New threats\\ identification\\ \textbullet Attack\\ surface area\\ \textbullet Develop\\ mitigation\\ techniques\end{tabular}} 
&          \\ \hline


\makecell {Chatterje,\\ Gupta, \\and De \\ \cite{chatterjee2013framework} \\(2013)}                  
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                          
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{}                                                                         
&            
&                                                                                                         
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Security\\ requirement:\\ \textbullet elicitation\\ \textbullet analysis\\ \textbullet prioritization\\ \textbullet  management\end{tabular}}                                                                      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Map security\\ requirements with\\ cryptographic\\ services\\ \textbullet Security design\\ analysis\\ \textbullet Security design\\ constraints\\ \textbullet Security design\\ structuring\\ \textbullet Security design\\ decisions\end{tabular}}                                                                               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Data protection\\ services\\ \textbullet Secure document\\ delivery\\ \textbullet Application\\ security\\ integration\\\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Vulnerability\\ scan\\ \textbullet Vulnerability\\assessment\\ \textbullet Security\\ assessment\\ \textbullet Security audit\\ and review\end{tabular}}                                                                    
& \multicolumn{1}{c|}{} 
&          \\ \hline


\makecell {Farhan \\ and\\ Mostafa\\ \cite{farhan2018methodology} \\(2018)}                      
& \multicolumn{1}{c|}{}                                                                
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}Developer\\ training\end{tabular}}                                                                         
&            
&  \begin{tabular}[c]{@{}l@{}}External\\ security\\ review\end{tabular}                                                                                              
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Application\\ portfolio analysis\\ \textbullet User risk analysis\\ \textbullet Architecture\\ risk analysis\end{tabular}}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Architecture\\ risk analysis\\\textbullet Design risk\\ analysis  \end{tabular}}                                                                                
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Coding standards\\ development\\ \textbullet Static code\\ analysis\end{tabular}}               
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Security metrics\\ development\\ \textbullet Test reviews\\ \textbullet Penetration\\ testing \end{tabular}}                                                                    
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\textbullet Penetration\\ testing\\ \textbullet Application\\ infrastructure\\ management\\ \textbullet Pre-implement\\ risk management\end{tabular}}                                                                     
&          \\ \hline
\end{longtable}
\end{landscape}







%The table for Agile methodologies
\begin{landscape}
\tiny % text size
\renewcommand{\arraystretch}{0.8}%for the length between lines
\setlength{\tabcolsep}{2pt}%the gap width of columns
\setlength\LTcapwidth{\textwidth} % default: 4in (rather less than \textwidth...)  
%\setlength\LTleft{0pt}            % default: \fill don't know use or not
%\setlength\LTright{0pt}           % default: \fill  don't know use or not
%\begin{longtable}{@{\extracolsep{\fill}}|c|ccccccc|c|cccccccc|} extracolsep adds a gab between lines. That's why I don't use it in this table
\begin{longtable}{|c|ccccccc|c|ccccccc|}
\caption{Summary of secure SDLC methodologies and involved secure practices for Agile development}
\label{tab:agile}\\ 
\hline
\multirow{3}{*}{Methodology} & \multicolumn{7}{c|}{Organizational-wide processes}  & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Processes\\ that\\ cover all\\ stages\\ of SDLC\end{tabular}} & \multicolumn{7}{c|}{\multirow{2}{*}{SDLC stages for a specific project}}\\ \cline{2-8} & \multicolumn{2}{c|}{Technical process}& \multicolumn{3}{c|}{Technical management process}
& \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Organizational processes\end{tabular}} &   & \multicolumn{7}{c|}{}  \\ \cline{2-8} \cline{10-16}  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}During \\ all \\ stages\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Preliminary\\ stages\\ for \\ maintenance\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Risk\\manage-\\ment\\frame-\\work\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Third\\party\\compo-\\nents\\manage-\\ment\end{tabular}} & \multicolumn{1}{c|}{Other} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Security\\ culture\end{tabular}}  & Other   &     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Project\\ inception\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Analysis \\ and \\ requirements\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Architectural \\ and detailed \\ design\end{tabular}} & \multicolumn{1}{c|}{Implementation} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Verification \\ and testing\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Release \\ and \\ maintenance\end{tabular}} & Disposal \\ \hline
%\endfirsthead % repeat header
%
\endhead
%


\makecell {SDL-Agile \\ \cite{whitepapermicrosoft}\\(2012)}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{blue!25}{Determine}\\\colorbox{blue!25}{security}\\\colorbox{blue!25}{response}\\\colorbox{blue!25}{standards}}}
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{}  
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} Security\\education\end{tabular}} 
&   
&   
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{blue!25}{\textbullet Identify}\\\colorbox{blue!25}{security and}\\ \colorbox{blue!25}{privacy}\\ \colorbox{blue!25}{expert}\\\colorbox{blue!25}{\textbullet Identify}\\\colorbox{blue!25}{primary}\\\colorbox{blue!25}{security}\\\colorbox{blue!25}{and privacy}\\\colorbox{blue!25}{contacts}\\\colorbox{red!25}{\textbullet Ensure all}\\ \colorbox{red!25}{team}\\ \colorbox{red!25}{members}\\\colorbox{red!25}{have had}\\\colorbox{red!25}{security}\\ \colorbox{red!25}{education}\\\colorbox{red!25}{within}\\ \colorbox{red!25}{the past}\\ \colorbox{red!25}{year}}}
& \multicolumn{1}{c|}{} 
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{red!25}{\textbullet Update the}\\ \colorbox{red!25}{threat model}\\ \colorbox{red!25}{\textbullet Communicate}\\ \colorbox{red!25}{privacy-impact}\\ \colorbox{red!25}{design changes}\\ \colorbox{red!25}{to the team}\\ \colorbox{red!25}{privacy advisor}\\ \colorbox{green!25}{\textbullet Design review}\\ \colorbox{blue!25}{\textbullet Baseline}\\\colorbox{blue!25}{threat model}\\\colorbox{blue!25}{\textbullet Threat model}\\\colorbox{blue!25}{your product,}\\\colorbox{blue!25}{its attack surface}\\\colorbox{blue!25}{and its new}\\\colorbox{blue!25}{features}}} 
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\colorbox{red!25}{\textbullet Security coding}\\ \colorbox{red!25}{standards}\\ \colorbox{blue!25}{\textbullet Security coding}\\ \colorbox{blue!25}{standards}\\\colorbox{red!25}{\textbullet Host security}\\ \colorbox{red!25}{deployment}\\ \colorbox{red!25}{review} \\\colorbox{red!25}{\textbullet Fix all issues}\\\colorbox{red!25}{identified by}\\\colorbox{red!25}{code analysis}\\\colorbox{red!25}{tools for}\\\colorbox{red!25}{unmanaged}\\\colorbox{red!25}{code}\end{tabular}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} \colorbox{green!25}{\textbullet Verification}\\\colorbox{green!25}{tasks}\end{tabular}}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}  \colorbox{red!25}{\textbullet Final}\\\colorbox{red!25}{security}\\\colorbox{red!25}{review}\\ \colorbox{green!25}{\textbullet Response}\\\colorbox{green!25}{planning}\end{tabular}} 
&  \\ 
\hline 


\makecell {GE\\ \cite{ge}\\ (Last\\access\\2022)}
& \multicolumn{1}{c|}{}
& \multicolumn{1}{c|}{}                                                                                  
& \multicolumn{1}{c|}{}                                                           
& \multicolumn{1}{c|}{}                                                                               
& \multicolumn{1}{c|}{}      
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\colorbox{green!25}{Developer}\\ \colorbox{green!25}{security}\\ \colorbox{green!25}{training}\end{tabular}}                                                                        
&            
&  \begin{tabular}[c]{@{}l@{}}Continuous\\ risk\\ assessment\end{tabular}                                                                                                       
& \multicolumn{1}{c|}{}                                                            
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}}\colorbox{blue!25}{\textbullet Review design}\\ \colorbox{blue!25}{\textbullet Provide}\\ \colorbox{blue!25}{security}\\ \colorbox{blue!25}{design input}\\  \colorbox{blue!25}{\textbullet Establish}\\ \colorbox{blue!25}{security}\\ \colorbox{blue!25}{user stories}\end{tabular}}                                                                 
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{red!25}{\textbullet Threat model}\\ \colorbox{red!25}{\textbullet Update security}\\ \colorbox{red!25}{user stories}\\ \colorbox{green!25}{\textbullet Update}\\ \colorbox{green!25}{threat model} \\ \colorbox{blue!25}{\textbullet Attack surface}\\ \colorbox{blue!25}{analysis review}\\ \colorbox{blue!25}{and reduction}}}                                                                                
& \multicolumn{1}{c|}{\makecell[l]{{\colorbox{red!25}{\textbullet SAST}}\\ \colorbox{red!25}{\textbullet DAST}\\ \colorbox{red!25}{\textbullet Open Source}\\ \colorbox{red!25}{vulnerability}\\\colorbox{red!25}{assessment}}}      
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{blue!25}{Penetration}\\ \colorbox{blue!25}{testing}}}                                                                 
& \multicolumn{1}{c|}{\makecell[l]{\colorbox{blue!25}{Update}\\ \colorbox{blue!25}{response}\\ \colorbox{blue!25}{services}}}                                   
&          \\ \hline

%row for the colors
\multicolumn{6}{|c|}{\colorbox{blue!25}{One time practices}}
& \multicolumn{5}{c|}{\colorbox{red!25}{Every sprint practices}}
& \multicolumn{5}{c|}{\colorbox{green!25}{Bucket practices}}\\

\hline

\end{longtable}
\end{landscape}
